Statistical limits of dictionary learning: random matrix theory and the spectral replica method

We consider increasingly complex models of matrix denoising and dictionary learning in the Bayes-optimal setting, in the challenging regime where the matrices to infer have a rank growing linearly with the system size. This is in contrast with most existing literature concerned with the low-rank (i.e., constant-rank) regime. We first consider a class of rotationally invariant matrix denoising problems whose mutual information and minimum mean-square error are computable using techniques from random matrix theory. Next, we analyze the more challenging models of dictionary learning. To do so we introduce a novel combination of the replica method from statistical mechanics together with random matrix theory, coined spectral replica method. This allows us to derive variational formulas for the mutual information between hidden representations and the noisy data of the dictionary learning problem, as well as for the overlaps quantifying the optimal reconstruction error. The proposed method reduces the number of degrees of freedom from $\Theta(N^2)$ matrix entries to $\Theta(N)$ eigenvalues (or singular values), and yields Coulomb gas representations of the mutual information which are reminiscent of matrix models in physics. The main ingredients are a combination of large deviation results for random matrices together with a new replica symmetric decoupling ansatz at the level of the probability distributions of eigenvalues (or singular values) of certain overlap matrices and the use of HarishChandra-Itzykson-Zuber spherical integrals.

==> sections/numerics.tex <==
\section{Numerically solving the Coulomb gases: a population dynamics approach}\label{sec:numerics}

We provide population dynamics schemes to solve the variational problems involved in the preceding conjectures. We also show that the minimum mean-square error (MMSE) can also be computed within this approach. Our goal here is not to be numerically sophisticated and we restrict ourselves to simple schemes. A jupyter notebook to run these various numerical experiments can be found here \cite{jupyter}.

\subsection{Warm up}
%
As a warm up consider first 
\begin{align*}
\tau_N&= -\sup_{\bLam^s\in\mathbb{R}^N} \Big\{\frac\beta2\sum_{i\neq j}^{1,N}\frac{\ln|\lambda^s_i-\lambda^s_j|}{N^2}-\frac\beta 4\sum_{i\le N}\frac{V({\lambda}^s_i)}{N}\Big\}
\end{align*}
which enters Result~\ref{conjectureHermitianRotInv}. This is simply the logarithm of the normalization constant of the j.p.d.f. of eigenvalues of a random matrix drawn according to $P_{S,N}$. Its stationary point(s) satisfy
%
\begin{align*}
\frac14V^\prime(\lambda_i^s) = R_{i,N}(\bLam^s) \quad \mbox{for}\quad i= 1, \dots, N
\end{align*}
where the ``resolvent'' $R_{i,N}:\mathbb{R}^N\mapsto \mathbb{R}$ is
%
\begin{align}
R_{i,N}(\bLam):=\frac1N\frac{\partial}{\partial \lambda_i}\ln \Delta(\bLam)= \frac{1}{N}\sum_{j:j\neq i}^{N-1}  \frac{1}{\lambda_i - \lambda_j}	. \label{R_i}
\end{align}
Note that $\partial_{\lambda_i}\ln |\Delta(\bLam)|=\partial_{\lambda_i}\ln \Delta(\bLam)$. A naive numerical scheme to solve this set of equations proceeds as follows. Take an initial set of random values $\bLam^{s, (0)}\in \mathbb{R}^N$ and fixed $g^{(-1)}_i=0$ for $i=1,\dots,N$, and iterate over $n=0,1,\dots$ in parallel over $i$:
\begin{align}\label{GDwarmup}
\begin{cases}
	g_i^{(n)} &= \gamma g_i^{(n-1)} + \eta\big(\frac14V^\prime(\lambda_i^{s, (n)}) - R_{i,N}(\bLam^s)\big)\\
\lambda_i^{s, (n+1)} &= \lambda_i^{s, (n)} - g_i^{(n)}	
\end{cases}
\quad \mbox{for}\quad i= 1, \dots, N 
\end{align}
% % 
% \begin{align*}
% \lambda_i^{s, (n+1)} = \lambda_i^{s, (n)} - \eta\Big(\frac14V^\prime(\lambda_i^{s, (n)}) - \frac{1}{N}\sum_{j:j\neq i}^{N} \frac{1}{\lambda_i^{s, (n)} - \lambda_j^{s, (n)}}\Big)\quad \mbox{for}\quad i= 1, \dots, N
% \end{align*}
% %
until convergence of the empirical distribution ${N^{-1}}\sum_{i\le N} \delta(x - \lambda_i^{s, (n)})$ of the population $\bLam^{s,(n)}$. It can be checked by tracking the convergence of some high enough moment of the empirical distribution. In practice the second moment seems sufficient. This is recognized as a gradient descent scheme with learning rate $\eta >0$ and a momentum term controlled by $\gamma\in[0,1)$ (typically, $\eta\le 10^{-4}$ and $\gamma\le 10^{-2}$ seem appropriate).
%


\begin{example}
The simplest example on which we can test this scheme is a standard Wigner matrix $\bS=\bS^\dagger\in \mathbb{K}^{N\times N}$ with $P_{S,N}(\bS)\propto \exp{\rm Tr}[-\frac {\beta N}4\bS^2]$ (i.e., $V(x) = x^2$ in our notations fixed by \eqref{P_SN}). The empirical distribution found by this iterative scheme converges (as $n,N\to+\infty$) to the Wigner semi-circle law as it should 
$$
\frac{1}{N}\sum_{i\le N} \delta(x - \lambda_i^s) \to \rho_{\rm W}(x) := \frac{\mathds{1}(-2\leq x \leq 2)}{2\pi}\sqrt{4 - x^2},
$$
(where $\mathds{1}(\cdot)$ is the indicator function) and this for any initial condition due to the convexity of the potential, provided $\eta$ is small enough.
\end{example}

\begin{example}
A second example is the Wishart matrix $\bS = \bX \bX^\dagger$ with $\bX\in \mathbb{K}^{N\times M}$ drawn from $P_{X,M}(\bX)\propto \exp{\rm Tr}[-\frac {\beta M}2\bX\bX^\dagger]$. Letting $\alpha:=N/M$ it induces the potential $V(x) = 2(1 - 1/\alpha) \ln\vert x\vert  +  2x/ \alpha$ in our notations fixed by \eqref{P_SN}, see e.g. \cite{potters2020first}. The empirical distribution found by this iterative scheme converges to the Marcenko-Pastur distribution of parameters $c:=(\sqrt\alpha -1)^2$ and $d:=(\sqrt\alpha +1)^2$
%
\begin{align*}
\frac{1}{N}\sum_{i\le N} \delta(x - \lambda_i^s) \to \rho_{\rm MP}(x) := \max(1-1/\alpha, 0) \delta(x) + \frac{\mathds{1}(c\leq x \leq d)}{2\pi \alpha x} 
\sqrt{(x - c)(d- x)} .
%\label{MPdistr}
\end{align*}
%
For $\alpha \le 1$ the potential is convex on $\mathbb{R}_{\ge 0}$ and convergence for any non-negative initial condition $\bLam^{s,(0)}\in \mathbb{R}^N_{>0}$ is guaranteed, provided $\eta$ is small enough. 
\end{example}

\subsection{Hermitian rotationally invariant denoising model}
%
We are concerned with solving the variational problem of conjecture \ref{conjectureHermitianRotInv}. 
The stationary point(s) satisfy equations \eqref{fpeq_1} for $i=1,\dots,N$ that we equivalently rewrite here for convenience when $\beta=2$:
\begin{align}
 \lambda\lambda_i^s+\frac{V'(\lambda^s_i)}{2}-2R_{i,N}(\bLam^s) - N\frac{\partial}{\partial \lambda^s_i} I_N^{(2)}(\bLam^s,\bLam^Y,\sqrt{\lambda})=0. \label{fpeq_1_bis}
\end{align}
In the Hermitian case $\beta =2$ we can use the exact Harish-Chandra-Itzykson-Zuber formula for $I^{(2)}_N(\bLam^s,\bLam^Y,\sqrt{\lambda})$, see the Appendix. For numerics it is useful to work with traceless matrices: let $\tilde \bLam^s:=\bLam^s-\theta_1^s$ where $\theta_1^s:= N^{-1}{\rm Tr}\bLam^s$ and similarly for $\tilde \bLam^Y$. Then
%
\begin{align*}
I_N^{(2)}(\bLam^s,\bLam^Y,\sqrt{\lambda})&=I_N^{(2)}(\tilde \bLam^s,\tilde \bLam^Y,\sqrt{\lambda})+\gamma \theta_1^s\,\theta_1^Y.
\end{align*} 
%
Recall that we equivalently denote $\bM=[M_{ij}]=[M_{cd}]=(M_{ij})_{i,j}=(M_{cd})_{c,d}$ for matrices, so in particular $[\exp{N\sqrt\lambda \lambda_c^s \lambda_d^Y}] := (\exp{N\sqrt\lambda \lambda_c^s \lambda_d^Y})_{c, d\leq N}$. Thus
\begin{align*}
-N\frac{\partial}{\partial \lambda_i^s} I_N^{(2)}( \bLam^s,\bLam^Y,\sqrt{\lambda} )
= \frac{1}{N}\frac{\partial}{\partial \lambda_i}\ln |\Delta(\bLam^s)|-\frac{1}{N} \frac{\partial}{\partial\lambda_i^s}\ln {\rm det}[\exp{N\sqrt\lambda \lambda_c^s \lambda_d^Y}]  .
\end{align*}
To compute the first derivative, we recall the Jacobi formula:
$$\frac{\partial}{\partial {X_{ij}}} \ln {\rm det} \bX = (\bX^{-1})_{ji}.$$
Then by an application of the chain rule we find for each $i=1, \dots, N$,
\begin{align*}
\frac1N\frac{\partial   }{\partial\lambda_i^s} \ln {\rm det} [\exp{N\sqrt\lambda \lambda_c^s \lambda_d^Y}]
& =
\frac1N\sum_{j\le N} \frac{\partial  \ln {\rm det} [\exp{N\sqrt\lambda \lambda_c^s \lambda_d^Y}]}{\partial\exp{N\sqrt\lambda \lambda_i^s \lambda_j^y}}  \frac{\partial \exp{N\sqrt\lambda \lambda_i^s \lambda_j^Y}}{\partial\lambda_i^s} \nonumber\\
&= 
\sum_{j\le N} ([\exp{N\sqrt\lambda \lambda_c^s \lambda_d^Y}]^{-1})_{ji} \sqrt\lambda  \lambda_j^Y \exp{N\sqrt\lambda \lambda_i^s \lambda_j^Y}, 
\end{align*}
where $[\exp N{\sqrt\lambda \lambda_c^s \lambda_d^Y}]^{-1}$ is a matrix inverse (of generalized Vandermonde type). For the second derivative recall formula \eqref{R_i}; this second derivative term will simplify with one resolvent in \eqref{fpeq_1_bis}.

Let $L_{i,N}(\cdot \mid \bLam^Y,\lambda):\mathbb{R}^N\mapsto \mathbb{R}$ be defined as
\begin{align*}
L_{i,N}(\bLam^s\mid \bLam^Y,&\lambda):= \lambda  \lambda_i^s + \frac{V'(\lambda_i^s)}{2} -R_{i,N}(\bLam^s)-  \sum_{j\le N}([\exp{N\sqrt\lambda \lambda_c^s \lambda_d^Y}]^{-1})_{ji} \sqrt\lambda  \lambda_j^Y \exp{N\sqrt\lambda \lambda_i^s \lambda_j^Y} .	
\end{align*}
% Then the fixed point(s) equations \eqref{fpeq_1} for the set of eigenvalues $\bLam^s$ become
% %
% \begin{align*}
% & L_{i,N}(\bLam^s\mid \bLam^Y,\lambda)=0\quad \mbox{for}\quad  i=1,\dots,N.
% \end{align*}
% %
It is numerically more efficient to work in vector form. Let
$L_{N}(\cdot \mid \bLam^Y,\lambda,m):\mathbb{R}^N\mapsto \mathbb{R}^N$ be
\begin{align*}
&L_{N}(\bLam^s\mid \bLam^Y,\lambda,m):=\Big(\lambda  \lambda_i^s + \frac{V'(\lambda_i^s)}{2}-R_{i,N}(\bLam^s)\Big)_{i\le N} \nonumber \\
&\qquad\qquad\qquad\qquad- {\rm sum}_{\rm col}\Big([\exp N({\sqrt\lambda \lambda_j^s \lambda_i^Y}-m)]^{-1}\odot [\sqrt\lambda  \lambda_j^Y \exp{N(\sqrt\lambda \lambda_i^s \lambda_j^Y}-m)]\Big),
\end{align*}
where $\odot$ is the Hadamard (entrywise) product, the operator ${\rm sum}_{\rm col}:\mathbb{R}^{a\times b}\mapsto \mathbb{R}^a$ (for generic $a,b$) sums over the columns of a matrix (note that the generalized Vandermonde matrix has been transposed before inversion), and $m$ is a free parameter that leaves invariant $L_{N}(\bLam^s\mid \bLam^Y,\lambda,m)$. Then the fixed point equations \eqref{fpeq_1_bis} for the eigenvalues $\bLam^s$ become $$L_{N}(\bLam^s\mid \bLam^Y,\lambda,m)=\boldsymbol{0}.$$
The introduction of $m$ is purely for the purpose of avoiding to deal with too large numbers. Let $m_{ij}:=\sqrt{\lambda} \lambda_i^s \lambda^Y_j$. One may then simply choose $m=N^{-2}\sum_{i,j}m_{ij}$ or $m= \rho \max_{i,j} m_{ij}+(1-\rho) \min_{i,j} m_{ij}$ for some $\rho\in[0,1]$.

A simple scheme to solve the fixed point equations is as follows: fix a large enough $N$ (but numerically tractable, say around $N=\Theta(10^2)$ or $\Theta(10^3)$) and generate a random instance of data $\bY$ according to the Hermitian denoising model \eqref{model-exactly}. Diagonalize $\bY$ in order to obtain its eigenvalues $\bLam^Y$. Now, initialize the population $\bLam^{s,(0)}\in\mathbb{R}^N$ and fix $\bg^{(-1)}=\boldsymbol{0}$. Then iterate over $n=0,1,\dots$ a parallel gradient descent scheme with learning rate $\eta >0$ and momentum $\gamma\in[0,1)$:
%
\begin{align*}
\begin{cases}
	m^{(n)}&=\rho \max_{i,j} \{\sqrt{\lambda} \lambda_i^s \lambda^Y_j\}+(1-\rho) \min_{i,j} \{\sqrt{\lambda} \lambda_i^s \lambda^Y_j\} \\
	\bg^{(n)} &= \gamma \bg^{(n-1)} + \eta L_{N}(\bLam^{s,(n)}\mid \bLam^Y,\lambda,m^{(n)})\\
\bLam^{s, (n+1)} &= \bLam^{s, (n)} - \bg^{(n)}
\end{cases}
\end{align*}
until convergence (again, this can be checked by tracking along the iterations the variation of the second moment of the population $\bLam^{s,(n)}$). We recall that the free entropy of the model is expected to be self-averaging with respect to $\bLam^Y$, so for large enough $N$ this scheme provides a reasonable approximation of the asymptotic $N\to+\infty$ free entropy. But in order to lower the fluctuations while remaining numerically tractable, this overall procedure can be repeated for multiple random independent instances of $\bY$ (and thus $\bLam^Y$) in order to average over it.


\noindent \emph{Br\'ezin-Hikami approximation for the low signal-to-noise ratio regime.} \ Given that the above schemes require the computation of (generalized) Vandermonde matrices, it is very unstable numerically and we did not succeed in going beyond population sizes of around $N=10$ without getting overflows. Here we propose another alternative based on a powerful expansion obtained by Hikami and Br\'ezin \cite{hikami2006wkb} which, surprisingly, seems not to have yet attracted the attention it deserves (see also appendix A of \cite{banerjee2021orthogonally}). They showed the formula 
%
\begin{align*}
I_N^{(1)}(\bLam^s,\bLam^Y,2\gamma/N)&=\frac1{N^2}\ln\int d\mu_N^{(1)}(\bU) \exp \gamma{\rm Tr}\, \big[{\bm U}^{\intercal} \bLam^s{\bm U}\bLam^Y\big]	\\
&= \frac1{N^2}\ln\Big(\exp\Big(\gamma\sum_{i\le N}\lambda^s_i\lambda_i^Y \Big) \prod_{i<j}^{1,N} \Big(1+\frac{2\gamma}N(\lambda^s_i-\lambda^s_j)(\lambda^Y_i-\lambda^Y_j)\Big)^{-1/2}\Big)+o_N(1)\\
&= \frac\gamma{N^2}\sum_{i\le N}\lambda^s_i\lambda_i^Y  -\frac1{2N^2}\sum_{i<j}^{1,N}\ln \Big(1+\frac{2\gamma}N(\lambda^s_i-\lambda^s_j)(\lambda^Y_i-\lambda^Y_j)\Big)+o_N(1)
\end{align*}
when restricted to the real case $\beta=1$ (for other values of $\beta$ their formula is less practical as it requires an additional sum over $N!$ permutations of one of the two sets of eigenvalues); here the eigenvalues are ordered as $\lambda^s_1>\lambda^s_2>\cdots>\lambda^s_N$ and similarly for $\bLam^Y$. This formula is valid only when $2\gamma(\lambda^s_i-\lambda^s_j)(\lambda^Y_i-\lambda^Y_j)<N$ for all $i<j$, see the appendix A of \cite{banerjee2021orthogonally}. If we rescale $\gamma\to \sqrt{\lambda} N/2$ it becomes
%
\begin{align*}
I_N^{(1)}(\bLam^s,\bLam^Y,\sqrt{\lambda})= \frac{\sqrt{\lambda}}{2N}\sum_{i\le N}\lambda^s_i\lambda_i^Y  -\frac1{N^2}\sum_{i\neq j}^{1,N}\ln \big(1+\sqrt{\lambda}(\lambda^s_i-\lambda^s_j)(\lambda^Y_i-\lambda^Y_j)\big)+o_N(1)
\end{align*}
and the validity criterion reads $\sqrt{\lambda}(\lambda^s_i-\lambda^s_j)(\lambda^Y_i-\lambda^Y_j)<1$, which will be verified for a sufficiently small signal-to-noise ratio $\lambda$ (given that the eigenvalues remain bounded and $O(1)$). In this case,
%
\begin{align}
-N\frac{\partial}{\partial \lambda_i^s} I_N^{(1)}( \bLam^s,\bLam^Y,\sqrt{\lambda} ) = \frac {2\sqrt{\lambda}}N \sum_{j:j\neq i}^{N-1}\frac{\lambda_i^Y-\lambda_j^Y }{1+\sqrt{\lambda}(\lambda_i^s-\lambda_j^s)(\lambda_i^Y-\lambda_j^Y)}-\frac{\sqrt{\lambda}}{2}\lambda_i^Y.
\end{align}
The fixed point equations when $\beta=1$ are
%
\begin{align*}
\frac{\lambda  \lambda^s_i}{2}  + \frac{V'(\lambda^s_i)}4-R_{i,N}(\bLam^s) - N\frac{\partial}{\partial \lambda^s_i} I_N^{(1)}(\bLam^s,\bLam^Y,\sqrt{\lambda})=0. 
\end{align*}
With the above simplifications valid for $\lambda\ll 1$, the ``gradient operator'' simply reads
\begin{align*}
L_{N}(\bLam^s\mid \bLam^Y,\lambda):=\Big(\frac{\lambda  \lambda^s_i}{2}  + \frac{V'(\lambda^s_i)}4- R_{i,N}(\bLam^s)+\frac{2\sqrt\lambda} N \sum_{j\le N}\frac{\lambda_i^Y-\lambda_j^Y}{1+\sqrt{\lambda}(\lambda_i^s-\lambda_j^s)(\lambda_i^Y-\lambda_j^Y)}-\frac{\sqrt{\lambda}}2\lambda_i^Y\Big)_{i\le N}
\end{align*}
to be plugged in the iterations over $n=0,1,\ldots$
\begin{align*}
\begin{cases}	
	\bg^{(n)} &= \gamma \bg^{(n-1)} + \eta L_{N}(\bLam^{s,(n)}\mid \bLam^Y,\lambda)\\
\bLam^{s, (n+1)} &= \bLam^{s, (n)} - \bg^{(n)}
\end{cases}
\end{align*}
with same initializations as before: $\bLam^{s,(0)}\in\mathbb{R}^N$ and $\bg^{(-1)}=\boldsymbol{0}$. Empirically, a good initialization is $\bLam^{s,(0)}=\bLam^Y$. As it should, when $\lambda=0$ the above operator matches the one appearing in \eqref{GDwarmup}.

\noindent \emph{Sampling the spherical integral.} \ The Itzykson-Zuber formula, see the Appendix, is exact for finite $N$ but extremely hard to compute numerically due to the precense of the determinants of matrices with exponentially large and small entries. Let us consider instead an approximation strategy based on sampling. Recall formula \eqref{IZhermitian}:
%
\begin{align}
I_N^{(\beta)}(\bLam^A,\bLam^B,\gamma):=\frac1{N^2}\ln\int d\mu_N^{(\beta)}(\bU) \exp \frac{\beta \gamma}2 N\sum_{i,j\le N}|{U}_{ji}|^2 \lambda^A_j\lambda^B_i \label{4bis}
\end{align}
from which we also get
%
\begin{align*}
\frac{\partial}{\partial \lambda^A_k}I_N^{(\beta)}(\bLam^A,\bLam^B,\gamma)=\frac{\beta \gamma}{2N}\frac{\int d\mu_N^{(\beta)}(\bU)  (\sum_{i}|{U}_{ki}|^2 \lambda^B_i) \exp \frac{\beta \gamma}2 N\sum_{i,j}|{U}_{ji}|^2 \lambda^A_j\lambda^B_i}{\int d\mu_N^{(\beta)}(\bU) \exp \frac{\beta \gamma}2 N\sum_{i,j}|{U}_{ji}|^2 \lambda^A_j\lambda^B_i}
\end{align*}
%
We can interpret this latter identity in two equivalent sampling interpretations. The ``naive sampling'' interpretation is 
%
\begin{align*}
\frac{\partial}{\partial \lambda^A_k}I_N^{(\beta)}(\bLam^A,\bLam^B,\gamma)=\frac{\beta \gamma}{2N}\frac{\mathbb{E}_{\bU\sim \mu_N^{(\beta)}}  (\sum_{i}|{U}_{ki}|^2 \lambda^B_i) \exp \frac{\beta \gamma}2 N{\rm Tr} [{\bm U}^{\dagger} \bLam^A{\bm U}\bLam^B]}{\mathbb{E}_{\bU\sim \mu_N^{(\beta)}} \exp \frac{\beta \gamma}2 N{\rm Tr} [{\bm U}^{\dagger} \bLam^A{\bm U}\bLam^B]}
\end{align*}
where $\bU$ is drawn according to the Haar measure $\mu_N^{(\beta)}(\bU)$. The smarter one is
%
\begin{align*}
\frac{\partial}{\partial \lambda^A_k}I_N^{(\beta)}(\bLam^A,\bLam^B,\gamma)= \frac{\beta \gamma}{2N}\mathbb{E}_{\bU\sim {\rm HCIZ}_N^{(\beta)}(\cdot\, \mid\, \bLam^A,\bLam^B,\gamma)}\sum_{i}|{U}_{ki}|^2 \lambda^B_i
\end{align*}
where the HCIZ measure is
%
\begin{align}
{\rm HCIZ}_N^{(\beta)}(\bU \mid \bLam^A,\bLam^B,\gamma) = \frac{\mu_N^{(\beta)}(\bU) \exp \frac{\beta \gamma}2 N{\rm Tr}[{\bm U}^{\dagger} \bLam^A{\bm U}\bLam^B]}{\int d\mu_N^{(\beta)}(\bU) \exp \frac{\beta \gamma}2 N{\rm Tr} [{\bm U}^{\dagger} \bLam^A{\bm U}\bLam^B]}	.
\end{align}
A very recent work has precisely considered the problem of efficiently sampling matrices according to this measure \cite{leake2021sampling}. 

We consider the naive strategy due to its simplicity and the fact that it not only allows us to compute the derivative of the HCIZ with respect to the eigenvalues, but also the HCIZ integral itself. In this scheme one samples a number $K$ of i.i.d. Haar matrices $\{\bU^1,\ldots,\bU^K\}$ from the orthogonal ($\beta=1$) or unitary ($\beta=2$) group; this is easily implemented by Gram-Schmidt from random gaussian matrices. The issue are the exponential-in-$N$ factors $$\exp N f_N^{(\beta)}(\bU):=\exp \frac{\beta \gamma}2 N{\rm Tr} \big[{\bm U}^{\dagger} \bLam^A{\bm U}\bLam^B\big]$$ appearing in the above expressions that lead to numerical overflows. A simple trick is to tilt the measure: using the empirical mean, 
%
\begin{align*}
\mathbb{E}_{\bU\sim \mu_N^{(\beta)}} g(\bU)\exp N f_N^{(\beta)}(\bU)	&\approx \frac1 K \sum_{k\le K} g(\bU^k)\exp N f_N^{(\beta)}(\bU^k)\\
&=\exp (Nm_N) \frac1 K \sum_{k\le K} g(\bU^k)\exp N(f_N^{(\beta)}(\bU^k)-m_N),
\end{align*}
where $m_N:=f_N^{(\beta)}(\bU^{k^*})$ with $k^*\in[K]$ corresponding to the index such that $f_N^{(\beta)}(\bU^{k^*})$ is maximum among all samples from the population (or for another appropriate choice $m_N$ such that numerical overflows are avoided). Using this simple idea we reach
%
\begin{align}
\frac{\partial}{\partial \lambda^A_j}I_N^{(\beta)}(\bLam^A,\bLam^B,\gamma)\approx \frac{\beta \gamma}{2N}\frac{  \sum_{k\le K}  (\sum_{i}|{U}_{ji}^k|^2 \lambda^B_i)\exp N(f_N^{(\beta)}(\bU^k)-m_N)}{ \sum_{k\le K}\exp N(f_N^{(\beta)}(\bU^k)-m_N)},
\end{align}
and for the HCIZ integral itself
%
\begin{align}
I_N^{(\beta)}(\bLam^A,\bLam^B,\gamma)\approx \frac {m_N}{N} +\frac1{N^2}\ln \frac1 K \sum_{k\le K}\exp (f_N^{(\beta)}(\bU^k)-m_N).
\end{align}

\subsubsection{Minimum mean-square error}
%
By the I-MMSE relation, the MMSE is directly proportional to $\frac{d f_N}{d\lambda}$. At the stationary point of the functional in conjecture 
\ref{conjectureHermitianRotInv}, this total derivative is computed by taking a partial derivative with respect to "explicit" the $\lambda$ dependence in the terms $\lambda \sum_i(\lambda_a^s)^2$ and in the eigenvalues $\lambda_a^Y$. The terms coming from the "implicit" dependence in the solutions $\lambda_a^s$ of the fixed point equation do not contribute. We have Form the HCIZ formula we get for $\beta =2$
%
\begin{align}\label{mmse1}
\frac{d f_N}{d\lambda} 
= - \frac{1}{2N}\sum_{a=1}^N (\lambda_a^s)^2 + \frac{\partial}{\partial\lambda} I_N^{(2)}(\lambda^s, \lambda^Y, \sqrt\lambda)
\end{align}
%
and from the HCIZ formula for $\beta =2$ (carefully taking into account the prefactor)
%
\begin{align*}
\frac{\partial}{\partial\lambda} I_N^{(2)}(\lambda^s, \lambda^Y, \sqrt\lambda) 
& = \frac{1}{2\sqrt\lambda} \frac{\partial}{\partial\sqrt\lambda} I_N^{(2)}(\lambda^s, \sqrt\lambda\lambda^Y, 1)
\\ \nonumber &
=
\frac{1}{2\sqrt\lambda} \frac{\partial}{\partial\sqrt\lambda} \ln {\rm det}[e^{ \lambda_c^s (\sqrt\lambda\lambda_d^Y)}] 
- 
\frac{1}{2\sqrt\lambda} \frac{\partial}{\partial\sqrt\lambda} \ln {\rm det}[(\sqrt\lambda\lambda_d^Y)^{c-1}] 
\\ \nonumber &
= \frac{1}{2\sqrt\lambda N^2}
\sum_{a, b=1}^N
\frac{\partial \ln {\rm det}[e^{ \lambda_c^s (\sqrt\lambda\lambda_d^y)}] }{\partial (e^{ \lambda_a^s (\sqrt\lambda\lambda_b^Y)})} 
\frac{\partial e^{ \lambda_a^s (\sqrt\lambda\lambda_b^Y)}}{\partial \sqrt\lambda}
\\ \nonumber &
- \frac{1}{2\sqrt\lambda N^2}
\sum_{a, b=1}^N \frac{\partial  \ln {\rm det}[(\sqrt\lambda\lambda_c^Y)^{d-1}]  }{\partial(\sqrt\lambda\lambda_a^Y)^{b-1}}
\frac{\partial  (\sqrt\lambda\lambda_a^Y)^{b-1}}{\partial \sqrt\lambda}
\nonumber \\ &
=
\frac{1}{2\sqrt\lambda N^2}\sum_{a, b=1}^N
[e^{ \lambda_c^s (\sqrt\lambda\lambda_d^y)}]^{-1}_{ba}   \lambda_a^s e^{ \lambda_a^s (\sqrt\lambda\lambda_b^Y)}
\frac{\partial (\sqrt\lambda\lambda_b^Y)}{\partial \sqrt\lambda}
\nonumber \\ &
- \frac{1}{2\sqrt\lambda N^2}
\sum_{a, b=1}^N ([(\sqrt\lambda\lambda_c^Y)^{d-1}]^{-1})_{ba}  (b-1) (\sqrt\lambda\lambda_a^Y)^{b-2} 
\frac{\partial(\sqrt\lambda\lambda_a^Y)}{\partial \sqrt\lambda}
\end{align*}
%
Now we need to compute derivatives of the spectrum $\frac{\partial (\sqrt\lambda\lambda_b^Y)}{\partial \sqrt\lambda}$. For this  we first note that 
$\frac{\partial (\sqrt\lambda\lambda_b^Y)}{\partial \sqrt\lambda} = \lambda_b^Y + \sqrt\lambda\frac{\partial \lambda_b^Y}{\partial \sqrt\lambda}$. The Hellmann-Feynman theorem implies $\frac{\partial \lambda_b^Y}{\partial \sqrt\lambda} = \langle \psi_b^Y \vert S \vert \psi_b^Y\rangle$ where 
$Y \vert \psi_b^Y\rangle = \lambda_b^Y \vert \psi_b^Y\rangle$, thus
% 
\begin{align*}
\frac{\partial (\sqrt\lambda\lambda_b^Y)}{\partial \sqrt\lambda}  = \langle \psi_b^Y \vert \sqrt\lambda S + \xi \vert \psi_b^Y\rangle + \sqrt\lambda \langle \psi_b^Y \vert S \vert \psi_b^Y\rangle = \langle \psi_b^Y \vert 2 \sqrt\lambda S + \xi \vert \psi_b^Y\rangle
\end{align*}
%
Putting everything together in \eqref{mmse1} we find 
\begin{align}\label{mmseresult}
\frac{d f_N}{d\lambda} 
= - \frac{1}{2N}\sum_{a=1}^N (\lambda_a^s)^2 
&
+ 
\frac{1}{2\sqrt\lambda N^2}\sum_{a, b=1}^N
[e^{ \sqrt\lambda \lambda_c^s\lambda_d^y}]^{-1}_{ba}   \lambda_a^s e^{ \sqrt\lambda\lambda_a^s \lambda_b^Y}
\langle \psi_b^Y \vert 2 \sqrt\lambda S + \xi \vert \psi_b^Y\rangle
\nonumber \\ &
- \frac{1}{2\sqrt\lambda N^2}
\sum_{a, b=1}^N ([(\sqrt\lambda\lambda_c^Y)^{d-1}]^{-1})_{ba}  (b-1) (\sqrt\lambda\lambda_a^Y)^{b-2} 
\langle \psi_a^Y \vert 2 \sqrt\lambda S + \xi \vert \psi_a^Y\rangle
\end{align}
%
We recall that  in this formula the eigenvalues $\lambda^s$ are to be understood as the solutions of teh fixed point equation \eqref{fixedpoint1}. We also observe that besides the matrix inversions this formula also requires to compute eigenvectors of $Y = \sqrt \lambda S + \xi$. We also note that it may be more practical to use $\langle \psi_a^Y \vert 2 \sqrt\lambda S + \xi \vert \psi_a^Y\rangle = \lambda_a^Y + \langle \psi_a^Y \vert \sqrt\lambda S\vert \psi_a^Y\rangle$.

